Mastering emergent language: learning to guide in simulated navigation

To cooperate with humans effectively, virtual agents need to be able to understand and execute language instructions. A typical setup to achieve this is with a scripted teacher which guides a virtual agent using language instructions. However, such setup has clear limitations in scalability and, more importantly, it is not interactive. Here, we introduce an autonomous agent that uses discrete communication to interactively guide other agents to navigate and act on a simulated environment. The developed communication protocol is trainable, emergent and requires no additional supervision. The emergent language speeds up learning of new agents, it generalizes across incrementally more difficult tasks and, contrary to most other emergent languages, it is highly interpretable. We demonstrate how the emitted messages correlate with particular actions and observations, and how new agents become less dependent on this guidance as training progresses. By exploiting the correlations identified in our analysis, we manage to successfully address the agents in their own language.

==> figures/guide-policy-exp-table.tex <==
\begin{table}[]
\begin{tabular}{L{0.3\linewidth}C{0.25\linewidth}C{0.25\linewidth}}
%{@{}lcc@{}}
\toprule
             & pretrained Guide + old policy & finetuned Guide + old policy \\ \midrule
GoToObj      & 99.8                          & $100.0 \pm 0.0$              \\
GoToLocal    & 94.7                          & $68.1 \pm 18.8$              \\
GoToObjMaze  & 91.6                          & $16.1 \pm 1.8$               \\
PickupLoc    & 93.4                          & $12.6 \pm 0.5$               \\
PutNextLocal & 73.0                          & $0.1 \pm 0.1$                \\
GoTo         & 37.9                          & $9.4 \pm 0.9$                \\ \bottomrule
\end{tabular}
\caption{Validation success rate (over 500 episodes) of the pretrained Guide with her own policy, and the finetuned Guide with the old policy (average over three runs with standard deviation).}
\label{tab:guide-policy-exp}
\end{table}


%gotoobj
%0.998
%1.0 1.0 1.0
%
%gotolocal
%0.947
%0.945 0.525 0.572
%
%gotoobjmaze
%0.916
%0.186 0.154 0.143
%
%pickuploc
%0.934
%0.131 0.119 0.129
%
%putnextlocal
%0.730
%0.000 0.002 0.000
%
%goto
%0.379
%0.107 0.088 0.086

==> figures/intralevel-table.tex <==
\begin{table}[h]
\begin{tabular}{L{0.3\linewidth}C{0.15\linewidth}C{0.4\linewidth}}
%{@{}ccc@{}}
\toprule
%             & \multicolumn{2}{c}{\begin{tabular}[x]{@{}c@{}}90\% validation success\\at epoch\end{tabular}} \\ \toprule
       & Learner            & Learner + pretrained Guide           \\ \midrule
GoToObj      & 10                 & 6                                    \\
GoToLocal    & 7                  & 2                                    \\
GoToObjMaze  & 5                  & 1                                    \\
PickupLoc    & 8                  & 1                                    \\
PutNextLocal & 14                 & 2                                    \\
GoTo         &  20                  &  12                                    \\ \bottomrule
\end{tabular}
\caption{Overview of number of training epochs required to reach a mean validation success rate of 90\% for a baseline Learner and a Learner assisted by a pretrained Guide.}
\label{tab:intralevel-success}
\end{table}
